Vocabulary Hijacking in LVLMs: Unveiling Critical Attention Heads by Excluding Inert Tokens to Mitigate Hallucination

Large Vision-Language Models (LVLMs) have achieved remarkable progress in multimodal tasks, yet their reliability is persistently undermined by hallucinations-generating text that contradicts visual input. Recent studies often attribute these errors to inadequate visual attention. In this work, we analyze the attention mechanisms via the logit lens, uncovering a distinct anomaly we term Vocabulary Hijacking. We discover that specific visual tokens, defined as Inert Tokens, disproportionately attract attention. Crucially, when their intermediate hidden states are projected into the vocabulary space, they consistently decode to a fixed set of unrelated words (termed Hijacking Anchors) across layers, revealing a rigid semantic collapse. Leveraging this semantic rigidity, we propose Hijacking Anchor-Based Identification (HABI), a robust strategy to accurately localize these Inert Tokens. To quantify the impact of this phenomenon, we introduce the Non-Hijacked Visual Attention Ratio (NHAR), a novel metric designed to identify attention heads that remain resilient to hijacking and are critical for factual accuracy. Building on these insights, we propose Hijacking-Aware Visual Attention Enhancement (HAVAE), a training-free intervention that selectively strengthens the focus of these identified heads on salient visual content. Extensive experiments across multiple benchmarks demonstrate that HAVAE significantly mitigates hallucinations with no additional computational overhead, while preserving the model's general capabilities. Our code is publicly available at https://github.com/lab-klc/HAVAE.

==> table/amber.tex <==
\begin{table*}[t]
\centering
\caption{
    AMBER benchmark results on LLaVA-1.5-7B. Best results are in \textbf{bold}. Superscripts show the \% change vs. the best baseline.
}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{ll|cccc|cc|c}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Model}}}
&\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}}
& \multicolumn{4}{c}{\textbf{Generative}} 
& \multicolumn{2}{c}{\textbf{Discriminative}} 
& \multicolumn{1}{c}{\textbf{AMBER}} \\ 
\cmidrule(lr){3-6} \cmidrule(lr){7-8} 
& & \textbf{CHAIR$_i$ $\downarrow$} & \textbf{Cover $\uparrow$}& \textbf{Hal $\downarrow$} & \textbf{Cog$^*$ $\downarrow$} &  \textbf{Acc. $\uparrow$}  & \textbf{F1 $\uparrow$} & \textbf{Score $\uparrow$} \\
\midrule
\multicolumn{1}{l}{\multirow{4}{*}{LLaVA-1.5-7B}} & Greedy        & 6.0 & 50.6 & 27.4 & 2.8 & 74.8 & 77.6 & 85.8 \\
& PAI               & 5.0 & 46.2 & 20.5 & 1.7 & 78.0 & 81.2 & 88.1 \\
& Devils            & 3.8 & 46.0 & 20.7 & \textbf{1.2} & 77.8 & 81.3 & 88.8 \\
& \textbf{HAVAE(Ours)} & \textbf{3.6}$^{\textcolor{mygreen}{\scriptsize -5.3\%}}$ & \textbf{51.7}$^{\textcolor{mygreen}{\scriptsize +2.2\%}}$ & \textbf{20.2}$^{\textcolor{mygreen}{\scriptsize -1.5\%}}$ & 1.3$^{\textcolor{myred}{\scriptsize +8.3\%}}$ & \textbf{78.6}$^{\textcolor{mygreen}{\scriptsize +0.8\%}}$ & \textbf{82.7}$^{\textcolor{mygreen}{\scriptsize +1.7\%}}$ & \textbf{89.6}$^{\textcolor{mygreen}{\scriptsize +0.9\%}}$ \\
\bottomrule
\end{tabular}
}

\label{tab:amber}
\end{table*}

==> table/hyper_set.tex <==
\begin{table}[t]
\centering
\caption{Hyperparameter settings.}
\label{tab:hyper_set}
\renewcommand{\arraystretch}{1.2} % Adds a bit of vertical spacing for readability
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{$\alpha$} & \textbf{$K$} & \textbf{$\tau$} & $|\hat{\mathcal{S}}|$ \\
\midrule
\textbf{LLaVA-1.5-7B}  & 0.6 & 450 & 23 & 10 \\
\textbf{MiniGPT-4-7B}  & 0.4 & 450 & 31 & 10 \\
\textbf{Shikra-7B}     & 0.7 & 450 & 32 & 1  \\
\textbf{LLaVA-1.5-13B} & 0.7 & 450 & 31 & 10 \\
\bottomrule
\end{tabular}
\end{table}

==> table/mme_and_qwen.tex <==
\begin{table*}[t]
\centering

% 左侧表格：旧模型的 MME 结果
\begin{minipage}[b]{0.40\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{l|cccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \textbf{LLaVA} & \textbf{MiniGPT-4} & \textbf{Shikra} & \textbf{LLaVA} \\
        & \textbf{1.5-7B} & \textbf{7B} & \textbf{7B} & \textbf{1.5-13B} \\
        \midrule
        \multicolumn{5}{c}{\textit{MME Perception}} \\
        Vanilla & 1472.5 & 731.9 & 962.0 & 1515.0 \\
        \textbf{Ours} & \textbf{1483.9} & \textbf{744.8} & \textbf{976.0} & \textbf{1528.9} \\
        \midrule
        \multicolumn{5}{c}{\textit{MME Cognition}} \\
        Vanilla & 322.5 & 173.0 & 250.4 & 290.6 \\
        \textbf{Ours} & \textbf{327.9} & \textbf{183.9} & \textbf{272.5} & \textbf{295.4} \\
        \bottomrule
        \end{tabular}
    }
    \caption{MME results on LLaVA, MiniGPT-4, and Shikra.}
    \label{tab:mme_baselines}
\end{minipage}
\hfill % 中间填充空隙
% 右侧表格：Qwen2-VL 的综合结果 (设置得更宽)
\begin{minipage}[b]{0.58\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{l|ccc|cc|cc}
        \toprule
        \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}} &
        \multicolumn{3}{c}{\textbf{CHAIR}} &
        \multicolumn{2}{c}{\textbf{POPE}} &
        \multicolumn{2}{c}{\textbf{MME}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        & \textbf{C$_s$ $\downarrow$} & \textbf{C$_i$ $\downarrow$} & \textbf{F1 $\uparrow$} & \textbf{Acc. $\uparrow$} & \textbf{F1 $\uparrow$} & \textbf{Per. $\uparrow$} & \textbf{Cog. $\uparrow$} \\
        \midrule
        Vanilla & 27.6 & 8.8 & 79.2 & 89.1 & 88.1 & 1700.2 & 568.2 \\
        \textbf{HAVAE} & \textbf{22.8} & \textbf{6.2} & \textbf{79.4} & \textbf{89.3} & \textbf{88.9} & \textbf{1711.6} & \textbf{578.6} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Results on Qwen2-VL across multiple benchmarks.}
    \label{tab:qwen_results}
\end{minipage}

\end{table*}

==> table/vista_pope.tex <==
\begin{table*}[t]
\centering
\caption{Performance of the VISTA method across different models and \(\lambda\) values.}
\label{tab:vista_ablation}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{ll|c|ccc|cc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\(\lambda\)}}} & \multicolumn{3}{c|}{\textbf{CHAIR}} & \multicolumn{2}{c}{\textbf{POPE}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-8}
& & & \textbf{CHAIRs} & \textbf{CHAIRi} & \textbf{F1} & \textbf{Acc} & \textbf{F1} \\
\midrule
\multirow{6}{*}{VISTA} & \multirow{2}{*}{LLaVA} & 0.01 & 48.4 & 13.2 & 75.9 & 83.1 & 84.6 \\
& & 0.17 & 15.6 & 5.2 & 67.3 & 56.7 & 63.3 \\
\cmidrule(lr){2-8}
& \multirow{2}{*}{MiniGPT-4} & 0.01 & 35.0 & 9.2 & 69.5 & 76.8 & 77.7 \\
& & 0.10 & 18.0 & 4.3 & 67.3 & 66.6 & 74.4 \\
\cmidrule(lr){2-8}
& \multirow{2}{*}{Shikra} & 0.01 & 55.2 & 15.1 & 74.0 & 82.4 & 82.4 \\
& & 0.12 & 32.8 & 9.8 & 73.4 & 79.0 & 76.8 \\
\bottomrule
\end{tabular}
}
\end{table*}
